Generalized Recognition of Basic Surgical Actions Enables Skill Assessment and Vision-Language-Model-based Surgical Planning

Artificial intelligence, imaging, and large language models have the potential to transform surgical practice, training, and automation. Understanding and modeling of basic surgical actions (BSA), the fundamental unit of operation in any surgery, is important to drive the evolution of this field. In this paper, we present a BSA dataset comprising 10 basic actions across 6 surgical specialties with over 11,000 video clips, which is the largest to date. Based on the BSA dataset, we developed a new foundation model that conducts general-purpose recognition of basic actions. Our approach demonstrates robust cross-specialist performance in experiments validated on datasets from different procedural types and various body parts. Furthermore, we demonstrate downstream applications enabled by the BAS foundation model through surgical skill assessment in prostatectomy using domain-specific knowledge, and action planning in cholecystectomy and nephrectomy using large vision-language models. Multinational surgeons' evaluation of the language model's output of the action planning explainable texts demonstrated clinical relevance. These findings indicate that basic surgical actions can be robustly recognized across scenarios, and an accurate BSA understanding model can essentially facilitate complex applications and speed up the realization of surgical superintelligence.

==> trajectoryplots/trajectoryplot.tex <==
\def\customlinethickness{0.8}
\def\custommarkersize{0.6}
\def\customendmarkersize{2.0}

\newcommand{\thumbnail}[2]{
    \begin{tikzpicture}
        \node (name) {#1};
        \node[anchor=west] at (name.east) {\includegraphics[width=0.5cm]{#2}};
    \end{tikzpicture}% <- this percentage sign actuall does something. Do not delete.
}
\pgfplotsset{
    myAxisStyle/.style={
    view={30}{20},
    unit vector ratio=1 1 1,
    scale=0.7,
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
    zticklabel style={font=\tiny},
    xtick distance=10,
    ytick distance=10,
    ztick distance=10,
    legend style={
        overlay,
        at={(0.5,2.5)},
        anchor=south,
        legend columns=4,
        font=\small,
        }, 
    }
}
\begin{figure}
\vspace{2cm}
\begin{tikzpicture}
\begin{axis}[
    name=firstClip,
    myAxisStyle
]
\input{trajectoryplots/plot_0}
\legend{};
\end{axis}

\begin{axis}[
    name=thirdClip,
    at=(firstClip.right of south east),
    anchor=left of south west,
    myAxisStyle
]
\input{trajectoryplots/plot_1}
\end{axis}

\begin{axis}[
    name=cut,
    at=(thirdClip.right of south east),
    anchor=left of south west,
    myAxisStyle
]
\input{trajectoryplots/plot_2}
\legend{};
\end{axis}

\node[below=5mm of firstClip] (FCT) {
\begingroup
\footnotesize
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{l c}
\textbf{SRT} \\
Duration (s): 18 & \\
Trajectory Length (mm): 31.387& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.544e^{-2}$ \\
\textbf{Surgeon}\\
Duration (s): 12 & \\
Trajectory Length (mm): 54.005& \\
Mean Jerk ($\frac{mm}{s^3}$): $3.058e^{-2}$ &
\end{tabular}
\endgroup
}; 
\node[below=2mm of FCT] {a) First clip}; 

\node[below=5mm of thirdClip] (TCT) {
\begingroup
\footnotesize
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{l c}
\textbf{SRT} \\
Duration (s): 25 & \\
Trajectory Length (mm): 43.450& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.675e^{-2}$ \\
\textbf{Surgeon} \\
Duration (s): 19 & \\
Trajectory Length (mm): 63.072& \\
Mean Jerk ($\frac{mm}{s^3}$): $3.050e^{-2}$ &
\end{tabular}
\endgroup
}; 
\node[below=2mm of TCT.south] {b) Third clip}; 

\node[below=5mm of cut] (CT) {
\begingroup
\footnotesize
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{l c}
\textbf{SRT} \\
Duration (s): 19 & \\
Trajectory Length (mm): 44.384& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.665e^{-2}$ \\
\textbf{Surgeon} \\
Duration (s): 13 & \\
Trajectory Length (mm): 47.348& \\
Mean Jerk ($\frac{mm}{s^3}$): $2.987e^{-2}$ &
\end{tabular}
\endgroup
}; 
\node[below=2mm of CT.south] {c) Cut}; 

\node[above=2mm of firstClip, anchor=south] (FC img) {\includegraphics[width=5cm]{trajectoryplots/firstclip.jpg}};
\node[above=2mm of thirdClip, anchor=south] (TC img) {\includegraphics[width=5cm]{trajectoryplots/thirdclip.jpg}};
\node[above=2mm of cut, anchor=south] (C img) {\includegraphics[width=5cm]{trajectoryplots/cut.jpg}};

\node[anchor=north east, xshift=-3mm] (A) at (FC img.north west) {\textbf{A}};
\node[anchor=north, below = 3.5cm of A] (B) {\textbf{B}};
\node[anchor=north, below = 3.25cm of B] {\textbf{C}};

\end{tikzpicture}
\caption{Text}

\end{figure}
